STAR-loc: Dataset for STereo And Range-based localization

This document contains a detailed description of the STAR-loc dataset. For a quick starting guide please refer to the associated Github repository (https://github.com/utiasASRL/starloc). The dataset consists of stereo camera data (rectified/raw images and inertial measurement unit measurements) and ultra-wideband (UWB) data (range measurements) collected on a sensor rig in a Vicon motion capture arena. The UWB anchors and visual landmarks (Apriltags) are of known position, so the dataset can be used for both localization and Simultaneous Localization and Mapping (SLAM).

==> _tables/rates.tex <==
\begin{tabular}{lrrrrr}
\toprule
topic & Apriltag & UWB & Vicon & IMU & duration [s] \\
dataset &  &  &  &  &  \\
\midrule
loop-2d\_s1 & 14.9 & 266.1 & 48.0 & 193.8 & 65.6 \\
loop-2d-fast\_s1 & 14.9 & 260.7 & 48.0 & 194.1 & 34.2 \\
loop-3d\_s1 & 14.9 & 249.3 & 48.0 & 193.6 & 87.7 \\
loop-2d\_s2 & 14.9 & 251.3 & 48.0 & 193.3 & 86.9 \\
loop-2d-fast\_s2 & 14.9 & 246.4 & 48.1 & 192.8 & 35.3 \\
loop-3d\_s2 & 14.9 & 244.6 & 48.0 & 192.6 & 80.3 \\
zigzag\_s2 & 14.9 & 256.4 & 48.0 & 193.0 & 78.0 \\
eight\_s2 & 15.0 & 246.6 & 48.1 & 192.3 & 49.2 \\
loop-2d\_s3 & 14.9 & 248.6 & 48.0 & 192.9 & 105.3 \\
loop-2d-fast\_s3 & 14.9 & 247.8 & 48.0 & 193.1 & 55.5 \\
loop-3d\_s3 & 14.9 & 249.4 & 48.0 & 193.9 & 99.8 \\
zigzag\_s3 & 14.9 & 249.4 & 48.0 & 193.9 & 201.6 \\
eight\_s3 & 14.9 & 247.4 & 48.0 & 192.9 & 98.5 \\
loop-2d\_s4 & 11.3 & 247.4 & 48.3 & 196.2 & 194.1 \\
zigzag\_s4 & 14.3 & 249.1 & 48.0 & 198.0 & 218.2 \\
grid\_s3 & 14.9 & 248.6 & 48.0 & 192.7 & 112.9 \\
ell\_s3 & 14.9 & 248.7 & 48.0 & 192.6 & 111.1 \\
loop-3d-z\_s3 & 14.9 & 249.1 & 48.0 & 193.2 & 150.3 \\
apriltag\_s3 & 14.9 & 247.8 & 48.0 & 193.1 & 116.4 \\
loop-2d\_s5 & 14.9 & 40.0 & 48.0 & 193.2 & 82.0 \\
loop-2d-v2\_s5 & 14.9 & 40.0 & 48.0 & 193.6 & 101.0 \\
loop-3d\_s5 & 14.9 & 40.0 & 48.0 & 193.1 & 67.0 \\
median rates [Hz] & 14.9 & 248.6 & 48.0 & 193.2 & nan \\
\bottomrule
\end{tabular}


==> _tables/times.tex <==
\begin{tabular}{lllr}
\toprule
 & start time & end time & duration [s] \\
dataset &  &  &  \\
\midrule
loop-2d-fast\_2tags-down\_v1 & 16:12:09 & 16:12:44 & 34.212641 \\
loop-2d\_2tags-down\_v1 & 16:13:31 & 16:14:37 & 65.582177 \\
loop-3d\_2tags-down\_v1 & 16:20:42 & 16:22:10 & 87.717770 \\
\bottomrule
\end{tabular}

